Learning Opinion Summarizers by Selecting Informative Reviews

Opinion summarization has been traditionally approached with unsupervised, weakly-supervised and few-shot learning techniques. In this work, we collect a large dataset of summaries paired with user reviews for over 31,000 products, enabling supervised training. However, the number of reviews per product is large (320 on average), making summarization - and especially training a summarizer - impractical. Moreover, the content of many reviews is not reflected in the human-written summaries, and, thus, the summarizer trained on random review subsets hallucinates. In order to deal with both of these challenges, we formulate the task as jointly learning to select informative subsets of reviews and summarizing the opinions expressed in these subsets. The choice of the review subset is treated as a latent variable, predicted by a small and simple selector. The subset is then fed into a more powerful summarizer. For joint training, we use amortized variational inference and policy gradient methods. Our experiments demonstrate the importance of selecting informative reviews resulting in improved quality of summaries and reduced hallucinations.

==> content/sections/old/subsampler.tex <==
 
 \section{Subsampler}
 
The central assumption is that the writer read a subset of reviews from the whole set that we have. And thus the actual reviews that were used to write the summary are latent, see Fig. \ref{fig:pgm}. 

Below we show the log-likelihood objective for one summary where we assume that $K$ reviewers were read out of $N$, where $K < N$.

\begin{equation}
\begin{aligned}
   &\log p_{\theta}(s | r_{1:N}) = \log \E_{r_{1:K} \sim p_{\theta}(r_{1:K} | r_{1:N})} \left[  p_{\theta}(s|r_{1:K}) \right]
\end{aligned}
 \end{equation}
 
 Here the prior $p_{\theta}(r_{1:K} | r_{1:N})$ serves as a bottle-neck that yields subsets of reviews $r_{1:K}$ out of the whole collection $r_{1:N}$. In other words, it captures that some reviews are more likely to be used for summarization by the writer. Intuitively, some might be uninformative and contain unique personal experiences unrepresentative of the population, and thus being less suitable for summarization. The other ones can be more aspect dense and thus are more suitable for summarization.
 
 To train the system, we derive the lower bound that uses the summary aware inference network as shown below. 
 
\begin{equation}
\begin{aligned}
  &\log \E_{r_{1:K} \sim p_{\theta}(r_{1:K} | r_{1:N})} \left[  p_{\theta}(s|r_{1:K}) \right] \geq \\ &\E_{r_{1:K} \sim q_{\phi}(r_{1:K}|r_{1:N}, s)} \left[ \log p_{\theta}(s|r_{1:K})\right] - \\ &\KL{q_{\phi}(r_{1:K}| r_{1:N}, s)}{p_{\theta}(r_{1:K}|r_{1:N})}
\end{aligned}
 \end{equation}
 
The approximate inference network $q_{\phi}(r_{1:K}| r_{1:N}, s)$ assigns probabilities to review subsets $r_{1:K}$ as if they had been read before the summary $s$ was written.
 
\subsection{Approximate posterior}
The approximate posterior can take a simpler form than the true posterior. The true posterior would require to marginalize over all the possible review subsets to perform normalization, see below.

\begin{equation}
    p_{\theta}(r_{1:K} | r_{1:N}, s) = \dfrac{ p_{\theta}(s|r_{1:K}) p_{\theta}(r_{1:K}| r_{1:N}) }{p_{\theta}(s | r_{1:N})}
\end{equation}

To avoid the computational burden, we assume a local factorization with a weak dependence on the previously selected reviews. 

\begin{equation}
    q_{\phi}(r_{1:K}|r_{1:N}, s) = \prod_{k=1}^K q_{\phi}(r_k|r_{1:N}, r_{1:{k-1}}, s)
\end{equation}

To compute the conditional distribution, we pass hand-crafted features such as ROUGE and AP through a FFNN to compute scores $f_{\phi}(s, r_k, r_{1:{k-1}})$. Then, we compute the distribution as below.

\begin{equation}
q_{\phi}(r_k|r_{1:N}, r_{1:{k-1}}, s) = \dfrac{\exp(f_{\phi}(s, r_k, r_{1:{k-1}}))}{\sum_{j=1}^N \exp(f_{\phi}(s, r_j, r_{1:{k-1}}))}
\end{equation}



Specifically, we compute distributions by blocking previously selected reviews. 

\subsection{Expectation}

Optimization of the lower bound is problematic specifically because of the expectation:

\begin{equation}
    \E_{r_{1:K} \sim q_{\phi}(r_{1:K}|r_{1:N}, s)} \left[ \log p_{\theta}(s|r_{1:K})\right]
\end{equation}

Which usually is approximated with MC sampling, where samples are obtained from the inference network.

The problem with this approach is that it requires to propagate gradients through a stochastic process, which is usually achieved via the re-parametrization trick. In its essence, the trick de-couples the parameters of the sample transformation from the noise sampled from a simple distribution. 

While this works for simple distributions such as Gaussian, which are easily re-parametrazible, it's unclear how to perform for the ones that are not. One such distribution is categorical, which is of our main interest. To avoid the hustle associated with Gumbel-softmax, we propose the following two options.

% \subsubsection{Noise distribution}

% \begin{equation}
% \begin{aligned}
%         &\E_{r_{1:K} \sim q_{\phi}(r_{1:K}|r_{1:N}, s)} \left[ \log p_{\theta}(s|r_{1:K})\right] = \\ &\E_{r_{1:K} \sim p(r_{1:K}|r_{1:N})} \left[ \dfrac{q_{\phi}(r_{1:K}|r_{1:N}, s)}{p(r_{1:K}|r_{1:N})}\log p_{\theta}(s|r_{1:K})\right]
% \end{aligned}
% \end{equation}

% Here, we have a simple noise distribution $p(r_{1:K}|r_{1:N})$, from which we can obtain samples. The important point is that it should be of the same type as $q_{\phi}(r_{1:K}|r_{1:N}, s)$. The important point is that it's not parametrized, and thus no updates are needed. 

% On the other hand, $q_{\phi}(r_{1:K}|r_{1:N}, s)$ changes its role from being a distribution for sampling to a being a distribution for sample weighting. The intuition is that the approximate posterior should assign higher probability to review samples $r_{1:K}$ that provide better signal for predicting $s$.

% Assuming that the noise distribution $p(r_{1:K}|r_{1:N})$ is equiprobable and that sampling is performed without replacement, then the factorization is the following.

% \begin{equation}
% \begin{aligned}
%     &p(r_{1:K}|r_{1:N}) = \prod_{k=1}^K p(r_k | r_{1:N-k}) = \\
%     &\prod_{k=1}^K \dfrac{1}{N-k+1} = \dfrac{(N-K)!}{N!}
% \end{aligned}
% \end{equation}

% Finally, we approximate the expectation term using MC, and arrive to the final equation below.
% \begin{equation}
% \begin{aligned}
%         &\E_{r_{1:K} \sim p(r_{1:K}|r_{1:N})} \left[ \dfrac{q_{\phi}(r_{1:K}|r_{1:N}, s)}{p(r_{1:K}|r_{1:N})}\log p_{\theta}(s|r_{1:K})\right] \approx \\
%         & \dfrac{N!}{(N-K)!} \prod_{k=1}^K q_{\phi}(r_k|r_{1:N}, s)\log p_{\theta}(s|r_{1:K})
% \end{aligned}
% \end{equation}

\subsubsection{REINFORCE}

The expectation estimate presented in the previous section has one downside. Namely, the samples are obtained from the prior noise distribution, which assuming to be equiprobable, can have very high variance, and thus resulting in a high variance gradient. An alternative is to obtain samples from the amortized posterior to approximate the expectation using REINFORCE.

The expectation with respect to the generative parameters is computed in the standard way as no backpropagation through samples is needed:

\begin{equation}
    \E_{r_{1:K} \sim q_{\phi}(r_{1:K}|r_{1:N}, s)} \left[ \nabla_{\theta} \log p_{\theta}(s|r_{1:K})\right].
\end{equation}

On the other hand, the gradient with respect to the variational parameters where REINFORCE is applied is shown below in a simplified notation.

\begin{equation}
    \begin{aligned}
        &\nabla_{\phi} \E_{r_{1:K} \sim q_{\phi}(\cdot)} \left[ \log p_{\theta}(s|r_{1:K})\right] = \\ &\E_{r_{1:K} \sim q_{\phi}(\cdot)} \left[ \nabla_{\phi} \log q_{\phi}(\cdot) (\log p_{\theta}(s|r_{1:K}) - \beta(s)) \right]
    \end{aligned}
\end{equation}

Here $\beta(s)$ corresponds to a baseline reducing the gradient variance \citep{sutton2018reinforcement}.

that should not depend on $r_{1:K}$, where the natural one would be $\E_{r_{1:K} \sim p_{\theta}(r_{1:K}|r_{1:N})} \left[ \log p_{\theta}(s|r_{1:K}) \right]$.


This makes sense from the perspective that we want to update proportionally to the improvement over a random draw from the prior.

% \subsubsection{Rescaling}

% Additionally, in order to promote selection of reviews that are better aligned to the summary, we can re-scale the reward using ROUGE F1 scores as shown below. 

% \begin{equation}
%     \E_{r_{1:K} \sim q_{\phi}(\cdot)} \left[ \nabla_{\phi} \log q_{\phi}(\cdot) R(s, r_{1:K})(\log p_{\theta}(s|r_{1:K}) - \beta(s)) \right]
% \end{equation}

% Assuming normalization by length, in the CLL, it makes sense to threat $R(s, r_{1:K})$ as the average ROUGE-1 score between the reviews and the summary:

% \begin{equation}
%     R(s, r_{1:K}) = \dfrac{1}{K} \sum_{k=1}^K ROUGE1(s, r_k)
% \end{equation}

\subsection{Kullback-Leibler divergence}


\subsubsection{Independent case}

Since we assumed that the reviews are independent, we can easily derive the KLD term as follows. 

\begin{equation}
\begin{aligned}
&\KL{q_{\phi}(r_{1:K}| r_{1:N}, s)}{p_{\theta}(r_{1:K}|r_{1:N})} = \\ &\sum_{k=1}^K \KL{q_{\phi}(r_k| r_{1:N}, s)}{p_{\theta}(r_k|r_{1:N})} = \\
&K\E_{q_{\phi}(r| r_{1:N}, s)}\left[ \log q_{\phi}(r| r_{1:N}, s)\right] - \\&K\E_{q_{\phi}(r| r_{1:N}, s)}\left[ \log p_{\theta}(r|r_{1:N}) \right] =\\
&- K  \mathbb{H}\left[ q_{\phi}(r| r_{1:N}, s)\right] - \\ & K \mathbb{CE}\left[q_{\phi}(r| r_{1:N}, s) || p_{\theta}(r|r_{1:N}) \right]
\end{aligned}
\end{equation}

\subsubsection{Conditional on history}

Here I assume that the current review depends on all previous reviews. The term will require approximation of the history, so we're technically talking about an estimate.

To make notation uncluttered, I make a couple of notion simplifications. $q_{\phi}(r_{1:K}| r_{1:N}, s) = q(r_{1:K})$, and same for the prior.

\begin{equation}
    \begin{aligned}
    &\KL{q(r_{1:K})}{p(r_{1:K})} = \E_{r_{1:K} \sim q(r_{1:K})}\left[ \log \dfrac{q(r_{1:K})}{p(r_{1:K})}\right] = \\
    &\sum_{k=1}^K \E_{r_{1:k-1} \sim q(r_{1:k-1})} \left[ \KL{q(r_k| r_{1:k-1})}{p(r_k| r_{1:k-1})} \right]
    \end{aligned}
\end{equation}

This can be approximated using one trajectory sample. First, we sample auto-regressively from $q(r_{1:K})$, then and then we approximate the term.

There are two case scenarios here. In the first one, we approximate the term for logging and gradients are not propagated. In the second scenario, we'll need to backpropagate the gradient through the system and thus REINFORCE will be needed. 

% \subsubsection{The old stuff}

% \begin{equation}
% \begin{aligned}
%     &\E_{r_{1:K} \sim q_{\phi}(r_{1:K}|r_{1:N}, s)} \left[ \log p_{\theta}(s|r_{1:K})\right] = \\ &\sum_{r_{1:K}} q_{\phi}(r_{1:K}|r_{1:N}, s) \log p_{\theta}(s|r_{1:K})
% \end{aligned}
% \end{equation}

% In the equation above, we scale conditional log-likelihoods by the probability of the samples $r_{1:K}$. And the sum is over all the possible samples. 

% Second, we split the sum into two parts:

% \begin{equation}
% \begin{aligned}
%     &\sum_{r_{1:K}} q_{\phi}(r_{1:K}|r_{1:N}, s) \log p_{\theta}(s|r_{1:K}) = \\ 
%     &\sum_{r_{1:K} \in M} q_{\phi}(r_{1:K}|r_{1:N}, s) \log p_{\theta}(s|r_{1:K}) + \\ 
%     &\sum_{r_{1:K} \in L} q_{\phi}(r_{1:K}|r_{1:N}, s) \log p_{\theta}(s|r_{1:K})
% \end{aligned}
% \end{equation}

% Here $M$ is a subset containing samples $r_{1:K}$ that we would like to explore, and $L$ are the ones that can be ignored. In the simplest scenario, we could sample units in $M$ or collect them  heuristically in the high probability area. Regardless of the collection procedure, it does not require to back propagate through samples as every possible sample $r_{1:K}$ can be either in $M$ or $L$.

% Next, we compute the approximate gradient by considering only the first sum. The idea is conceptually similar to Taylor expansion with consideration of linear terms only that are easy to compute.

% \begin{equation}
% \begin{aligned}
%     &\sum_{r_{1:K} \in M \cup L} \nabla q_{\phi}(r_{1:K}|r_{1:N}, s) \log p_{\theta}(s|r_{1:K}) \approx \\ 
%     &\sum_{r_{1:K} \in M}  \nabla  q_{\phi}(r_{1:K}|r_{1:N}, s) \log p_{\theta}(s|r_{1:K})
% \end{aligned}
% \end{equation}

% The gradient approaches the true one as we decrease the size of the left-out subset: $|L| \rightarrow 0$.


==> content/sections/rouge_topk_subs.tex <==
\section{ROUGE-based Subsampler}
\label{sec:rouge_topk_subsampler}

% The first subsampler is a special case where the approximate posterior has no trainable parameters. Instead, it uses a static score function based on ROUGE-1 F1. It follows intuition that more relevant reviews have a higher word overlap with the summary. In addition, it's a common heuristic in extractive summarization to select relevant sentences to the summary \citep{nallapati2016summarunner, liu2019text}. 

% However, ROUGE being an unweighted word overlap score, fails to down-weight uninformative reviews that use the same conjunction words and stylistic phrases as the summary. And as we sample subsets from the posterior, this results in such reviews appearing in reduced subsets. To alleviate this problem, we produce a degenerate distribution $q^{RG}(\hat{r}_k|r_{1:N}, \hat{r}_{1:k-1}, s)$ where all probability mass is allocated to one review that is the most likely.

% As the posterior has no trainable parameters, the Kullback-Leibler term is a constant cancelled by the derivative. And thus, we can maximize the reconstruction term in solely. Also, as all of the probability mass is allocated to one reduced collection of reviews $\hat{r}_{1:K}$, the reconstruction term can be computed without approximations with one single subset $\hat{r}_{1:K}^*$ greedy selected from the degenerate posterior as shown in Eq.~\ref{eq:lower_bound_greedy}. We refer to this subsampler as \textsc{ROUGE greedy}.


% \begin{equation}
% \begin{aligned}
%   &\log p_{\theta}(s| r_{1:N}) \geq \\ &\E_{\hat{r}_{1:K} \sim q^{RG}(\hat{r}_{1:K}|r_{1:N}, s)} \left[ \log p_{\theta}(s|\hat{r}_{1:K})\right] - C  &= \\
%   &\log p_{\theta}(s|\hat{r}_{1:K}^*) - C
%     \label{eq:lower_bound_greedy}
% \end{aligned}
% \end{equation}

% By no surprise, ROUGE is not an optimal metric for scoring alignment between documents \citep{tay2019red,kryscinski2019evaluating}. In addition, it is not trivially extensible to multiple features, which would require tuning efforts to weight them. Finally, it assumes a linear mapping from features to scores and complex features can require a non-linear mapping. Therefore, in Sec.~\ref{sec:var_subsampler}, we propose an approach that is extensible and uses a trainable non-linear mapping function.



==> content/summs/front.tex <==
% \textcolor{red}
% \textcolor{orange}
% \textcolor{blue}
% \textcolor{cyan}
% \textcolor{myGreen}
% B009L0KU46

\begin{table}[t!]
    \centering
 	\footnotesize 
    \begin{tabular}{ >{\centering\arraybackslash} m{1cm} m{5cm}} 
    \hline
    \textbf{Verdict} & \vspace{1.0em} \vspace{1.em} \\ \hline
    \textbf{Pros} & \vspace{1.em}  
        $\color{green}{\bullet}$\hspace{0.25em} \newline
        \vspace{1.0em}  \\ \hline
  \textbf{Cons} & \vspace{1.em} 
  $\color{red}{\bullet}$ \hspace{0.25em} \newline
  \vspace{1.0em}  \\ \hline
    \end{tabular}
    \caption{Example summaries for a squirrel feeder.}
    \label{table:front-example-summ-0}
\end{table}


==> content/summs/front1.tex <==
% \textcolor{red}
% \textcolor{orange}
% \textcolor{blue}
% \textcolor{cyan}
% \textcolor{myGreen}
% B009L0KU46

\begin{table}[t!]
    \centering
 	\footnotesize 
    \begin{tabular}{ >{\centering\arraybackslash} m{1cm} m{5cm}} 
    \hline
    \textbf{Verdict} & \vspace{1.0em} If you're looking for a reliable, water-resistant, and weather-resistant G-Shock watch, this is the one to get. \vspace{1.em} \\ \hline
    \textbf{Pros} & \vspace{1.em}  
        $\color{green}{\bullet}$ Solar powered\hspace{0.25em} \newline
        $\color{green}{\bullet}$ Water-resistant  \hspace{0.25em} \newline
        $\color{green}{\bullet}$ Includes atomic clock and countdown timer \hspace{0.25em} \newline
        $\color{green}{\bullet}$ Includes a stopwatch and 5 alarms \hspace{0.25em} 
        
        \vspace{1.0em}  \\ \hline
  \textbf{Cons} & \vspace{1.em} 
  
  $\color{red}{\bullet}$ Some owners say the watch is too small for their needs \hspace{0.25em} \newline
  $\color{red}{\bullet}$ A few owners say it doesn't have the features of other models \hspace{0.25em}
  \vspace{1.0em}  \\ \hline
    \end{tabular}
    \caption{Example summaries for a squirrel feeder.}
    \label{table:front-example-summ}
    \NoGap
\end{table}

